SABET-QA: Temporal Knowledge Graph Question Answering

Question Answering over Temporal Knowledge Graphs (TKGQA) requires reasoning over time-sensitive facts, yet existing embedding-based methods struggle with multi-step queries due to single-pass reasoning pipelines. We propose SABET-QA, a framework that iteratively refines reasoning states across multiple hops via a bidirectional entity-temporal scoring mechanism and a slot-aware contextualization module that aligns question semantics with temporal KG embeddings. A differentiable working memory enables progressive hypothesis refinement, while auxiliary temporal boundaries serve as coarse supervision when available. Experiments on CronQuestions, Complex-CronQuestions, MultiTQ, and TimeQuestions demonstrate consistent improvements over strong baselines, particularly on complex multi-step temporal queries.

==> components/4_theoretical_analysis.tex <==
\label{sec:theoretical_analysis}


==> components/acknowledgements.tex <==

Generative AI tools, including OpenAI's GPT models and Anthropic's Claude, were used in the writing process of this paper. These tools were employed to improve grammar or refine style and phrasing.

==> components/imsabt.tex <==
\subsection{Proposed Method: Iterative Multi-Hop Set-Aware Bidirectional Temporal Question Answering (IMSABT-QA)}

IMSABT-QA is an iterative temporal question answering model that combines pretrained language representations with temporal knowledge graph embeddings. The model is designed to answer questions by progressively refining its latent reasoning state over multiple hops. At each hop, IMSABT-QA constructs a hop-specific relation representation, computes entity and timestamp scores, and updates its internal state using the predicted answer distributions. This iterative process allows the model to revisit the question evidence multiple times and refine its prediction gradually.

% \subsubsection{Question encoding}

% Given a tokenized question $\mathbf{x} = (x_1,\dots,x_L)$ and its attention mask $\mathbf{m}$, IMSABT-QA first encodes the question with a pretrained language model:
% \[
% \mathbf{H} = \mathrm{LM}(\mathbf{x}, \mathbf{m}) \in \mathbb{R}^{L \times 768}.
% \]
% The contextual token states are then projected into the temporal knowledge graph embedding space:
% \[
% \mathbf{T} = f_{\text{text}}(\mathbf{H}) \in \mathbb{R}^{L \times D},
% \]
% where $D$ is the embedding dimension of the temporal KG model.

% When entity-aware annotations are available, structured temporal KG embeddings are injected into the token sequence at the corresponding positions. Let $\mathbf{P} \in \mathbb{R}^{L \times D}$ denote the projected entity/time embeddings aligned with the question tokens. The final token representation is obtained by combining the language representation with the structured signal:
% \[
% \tilde{\mathbf{T}} = \mathbf{T} + \mathbf{P}.
% \]
% This mechanism grounds the question representation in the temporal KG embedding space and provides an explicit bridge between text and symbolic knowledge.


% \subsubsection{Slot contextualization}

% IMSABT-QA represents the head, tail, and timestamp slots with embeddings $\mathbf{e}_h$, $\mathbf{e}_t$, and $\mathbf{e}_\tau$. These slot embeddings are contextualized by using them as queries in a multi-head attention block over the question tokens:
% \[
% \mathbf{C} = \mathrm{Attn}([\mathbf{e}_h;\mathbf{e}_t;\mathbf{e}_\tau], \tilde{\mathbf{T}}, \tilde{\mathbf{T}}).
% \]
% The output is normalized and combined with the original slot embeddings through a gated residual update, producing contextualized slot states
% \[
% \hat{\mathbf{e}}_h,\ \hat{\mathbf{e}}_t,\ \hat{\mathbf{e}}_\tau.
% \]
% This step aligns the entity and temporal slots with the semantics of the question while preserving the structural prior encoded by the temporal KG.


\subsubsection{Question encoding and entity-aware grounding}

Given a tokenized question $\mathbf{x}=(x_1,\dots,x_L)$ and attention mask $\mathbf{m}$, IMSABT-QA first encodes the question using a pretrained language model:
\[
\mathbf{H}=\mathrm{LM}(\mathbf{x},\mathbf{m})
\in\mathbb{R}^{L\times768}.
\]

The contextual token representations are projected into the temporal knowledge graph (TKG) embedding space:
\[
\mathbf{T}=f_{\text{text}}(\mathbf{H})
\in\mathbb{R}^{L\times D},
\]
where $D$ denotes the embedding dimension of the temporal KG model.

When entity-aware annotations are available, aligned entity and timestamp identifiers are mapped to their corresponding TKG embeddings:
\[
\mathbf{E}\in\mathbb{R}^{L\times D}.
\]
These embeddings are obtained from a shared entity--time embedding table initialized from the pretrained TKG model. Let
\[
\mathbf{M}\in\{0,1\}^{L}
\]
denote a binary mask indicating whether a token corresponds to a regular textual token or an aligned entity/time mention. The grounded token representation is computed as
\[
\tilde{\mathbf{T}}
=
\mathbf{T}
+
(1-\mathbf{M})\odot \mathbf{E},
\]
where $\odot$ denotes element-wise masking with broadcasting over the embedding dimension.

Unlike replacement-based grounding approaches, IMSABT-QA preserves the original contextual language representation and injects symbolic temporal KG information additively. This enables the model to jointly exploit linguistic context and structured temporal semantics within a shared embedding space.

\subsubsection{Slot contextualization}

IMSABT-QA represents the head, tail, and timestamp slots using embeddings retrieved from the same shared entity--time embedding space:
\[
\mathbf{e}_h,\qquad
\mathbf{e}_t,\qquad
\mathbf{e}_\tau.
\]

These slot embeddings are contextualized through multi-head cross-attention over the grounded question representation:
\[
\mathbf{C}
=
\mathrm{Attn}
\big(
[\mathbf{e}_h;\mathbf{e}_t;\mathbf{e}_\tau],
\tilde{\mathbf{T}}
\big).
\]

The resulting contextual slot states
\[
\mathbf{c}_h,\qquad
\mathbf{c}_t,\qquad
\mathbf{c}_\tau
\]
are normalized and fused with the original slot embeddings using gated residual updates:
\[
\mathbf{g}_h
=
\sigma\!\left(
W_g[\mathbf{e}_h;\mathbf{c}_h]
\right),
\]
\[
\hat{\mathbf{e}}_h
=
\mathbf{g}_h\odot\mathbf{e}_h
+
(1-\mathbf{g}_h)\odot\mathbf{c}_h,
\]
with analogous updates for the tail and timestamp slots.

This mechanism allows the slot representations to selectively integrate contextual evidence from the question while preserving the structural priors encoded by the temporal KG embeddings.

\paragraph{Architecture note.}
Figure~\ref{fig:sabtqa_text_slots} illustrates the joint question grounding and slot contextualization stage. In contrast to LM-only baselines, IMSABT-QA explicitly injects pretrained temporal KG embeddings into aligned token positions and contextualizes symbolic role embeddings through cross-attention with the grounded question representation.



\subsubsection{Global question summary}

In parallel, IMSABT-QA builds a global representation of the question using three complementary pooling operations: the \texttt{[CLS]} token, masked mean pooling, and masked max pooling. These vectors are concatenated and projected to obtain the summary representation
\[
\mathbf{s} = f_{\text{sum}}([\mathbf{T}_{\text{CLS}};\ \mathrm{Mean}(\tilde{\mathbf{T}});\ \mathrm{Max}(\tilde{\mathbf{T}})]) \in \mathbb{R}^{D}.
\]
This summary serves as a compact question-level context for relation construction, hop-specific projection, and final hop weighting.

\subsubsection{Initial relation refinement}

IMSABT-QA first constructs an initial relation representation by combining the global question summary with the contextualized head, tail, and temporal slot embeddings:
\[
\mathbf{r}_{\text{base}}
=
f_{\text{rel}}
\big(
[\mathbf{s};
\hat{\mathbf{e}}_h;
\hat{\mathbf{e}}_t;
\hat{\mathbf{e}}_\tau]
\big)
\in\mathbb{R}^{D},
\]
where $f_{\text{rel}}$ is a multilayer projection network.

Rather than directly using this vector for reasoning, IMSABT-QA refines it through a relation-aware cross-attention operation over the grounded question representation. Specifically, the initial relation vector is used as the query, while the grounded token representations act as keys and values:
\[
\mathbf{r}_{\text{ctx}}
=
\mathrm{Attn}
\big(
\mathbf{r}_{\text{base}},
\tilde{\mathbf{T}},
\tilde{\mathbf{T}}
\big).
\]

The resulting contextual relation state is integrated with the original relation vector using a residual connection followed by layer normalization:
\[
\mathbf{r}_{\text{ref}}
=
\mathrm{LayerNorm}
\big(
\mathbf{r}_{\text{base}}
+
\mathbf{r}_{\text{ctx}}
\big).
\]

This refinement stage allows the latent relation representation to dynamically re-attend to the question tokens after slot contextualization has already been performed. Consequently, the refined relation vector captures both global question semantics and token-level evidence relevant to the current entity and temporal roles.

The refined relation representation $\mathbf{r}_{\text{ref}}$ serves as the initial latent reasoning state for the subsequent multi-hop inference process:
\[
\mathbf{z}^{(0)}=\mathbf{r}_{\text{ref}}.
\]

\subsubsection{Hop-specific relation projection}

Starting from the refined latent reasoning state
\[
\mathbf{z}^{(0)}=\mathbf{r}_{\text{ref}},
\]
IMSABT-QA performs iterative multi-hop reasoning over $K$ hops. At each hop $k$, the current latent state $\mathbf{z}^{(k-1)}$ is concatenated with the global question summary $\mathbf{s}$ and transformed through a hop-specific projection network:
\[
\mathbf{r}^{(k)}
=
f_k
\big(
[\mathbf{z}^{(k-1)};\mathbf{s}]
\big),
\]
where $\{f_k\}_{k=1}^{K}$ are independent multilayer projection functions.

Unlike shared-hop architectures, IMSABT-QA allocates a distinct projection module to each reasoning step, allowing different hops to specialize in different reasoning patterns and temporal dependencies. The hop-specific relation representation is then decomposed into separate entity-oriented and time-oriented relation views:
\[
\mathbf{r}_{\text{ent}}^{(k)}
=
g_{\text{ent}}
\big(
\mathbf{r}^{(k)}
\big),
\qquad
\mathbf{r}_{\text{time}}^{(k)}
=
g_{\text{time}}
\big(
\mathbf{r}^{(k)}
\big),
\]
where $g_{\text{ent}}(\cdot)$ and $g_{\text{time}}(\cdot)$ denote dedicated projection networks for entity and temporal reasoning, respectively.

The entity-oriented relation representation is optimized for bidirectional entity scoring, while the temporal-oriented representation specializes in timestamp prediction and set-aware temporal reasoning. This factorization enables the model to disentangle structural entity interactions from temporal dynamics within each reasoning hop.

After computing entity and temporal scores, IMSABT-QA converts the resulting distributions into soft memory representations that are used to update the latent reasoning state for the next hop. Consequently, each reasoning step progressively refines the model's internal hypothesis based on previously inferred entity and temporal evidence.

Figure~\ref{fig:horizon_hops} illustrates the iterative hop-wise reasoning mechanism in IMSABT-QA.

\subsubsection{Bidirectional entity scoring}

At each reasoning hop, IMSABT-QA computes entity prediction scores using a TComplEx-style temporal scoring function parameterized by the hop-specific entity-oriented relation representation $\mathbf{r}_{\text{ent}}^{(k)}$. Given the contextualized head, tail, and temporal slot embeddings
\[
\hat{\mathbf{e}}_h,\qquad
\hat{\mathbf{e}}_t,\qquad
\hat{\mathbf{e}}_\tau,
\]
the model evaluates candidate entities in both forward and backward directions.

The forward score uses the original head--tail ordering:
\[
s_{\text{ent}}^{\rightarrow (k)}
=
\mathrm{Score}_{\text{TComplEx}}
\big(
\hat{\mathbf{e}}_h,
\hat{\mathbf{e}}_t,
\mathbf{r}_{\text{ent}}^{(k)},
\hat{\mathbf{e}}_\tau
\big),
\]
while the backward score swaps the head and tail roles:
\[
s_{\text{ent}}^{\leftarrow (k)}
=
\mathrm{Score}_{\text{TComplEx}}
\big(
\hat{\mathbf{e}}_t,
\hat{\mathbf{e}}_h,
\mathbf{r}_{\text{ent}}^{(k)},
\hat{\mathbf{e}}_\tau
\big).
\]

This bidirectional formulation enables the model to reason flexibly about temporal relations whose semantic direction may be ambiguous or implicitly expressed in natural language questions.

The two directional scores are combined using an adaptive fusion gate conditioned on the global question summary:
\[
\alpha^{(k)}
=
\sigma
\big(
W_{\text{bi}}\mathbf{s}
\big),
\]
\[
s_{\text{ent}}^{(k)}
=
\alpha^{(k)}
\,
s_{\text{ent}}^{\rightarrow (k)}
+
\big(
1-\alpha^{(k)}
\big)
s_{\text{ent}}^{\leftarrow (k)}.
\]

Unlike fixed averaging schemes, the learned gate allows IMSABT-QA to dynamically control the relative contribution of forward and backward reasoning pathways according to the semantics of the question.

\subsubsection{Set-aware temporal scoring}

Temporal prediction is performed using a TComplEx-based temporal scoring function augmented with a set-aware temporal reasoning mechanism. At hop $k$, the model first computes a base score distribution over candidate timestamps:
\[
s_{\text{time}}^{\text{base},(k)}
=
\mathrm{Score}_{\text{time}}
\big(
\hat{\mathbf{e}}_h,
\hat{\mathbf{e}}_t,
\mathbf{r}_{\text{time}}^{(k)}
\big).
\]

The resulting scores are converted into a soft temporal distribution:
\[
\mathbf{w}^{(k)}
=
\mathrm{Softmax}
\left(
\frac{
s_{\text{time}}^{\text{base},(k)}
}{
\tau
}
\right),
\]
where $\tau$ is a learned temperature parameter controlling the sharpness of the temporal distribution.

The soft distribution is then used to compute a weighted temporal summary over the full timestamp embedding table:
\[
\bar{\mathbf{t}}^{(k)}
=
\sum_j
w_j^{(k)}
\mathbf{t}_j.
\]

This temporal summary is projected back into the hidden space:
\[
\mathbf{u}^{(k)}
=
f_{\text{set}}
\big(
\bar{\mathbf{t}}^{(k)}
\big),
\]
and rescored against all timestamp embeddings to obtain a set-aware temporal score:
\[
s_{\text{time}}^{\text{set},(k)}
=
\mathbf{u}^{(k)}
\mathbf{T}^{\top},
\]
where $\mathbf{T}$ denotes the matrix of timestamp embeddings.

Finally, the base and set-aware temporal scores are combined using a learned gating mechanism:
\[
\lambda^{(k)}
=
\sigma
\left(
W_{\lambda}
[
\bar{\mathbf{t}}^{(k)};
\mathbf{s}
]
\right),
\]
\[
s_{\text{time}}^{(k)}
=
s_{\text{time}}^{\text{base},(k)}
+
\lambda^{(k)}
s_{\text{time}}^{\text{set},(k)}.
\]

This set-aware mechanism enables IMSABT-QA to capture temporally distributed evidence and compositional temporal constraints that cannot be adequately represented by a single timestamp prediction.

\subsubsection{Working-memory update}

After obtaining hop-specific entity and temporal scores, IMSABT-QA updates its latent reasoning state using a differentiable working-memory mechanism. The hop-level entity and temporal scores are first normalized into probability distributions:
\[
\mathbf{p}^{(k)}
=
\mathrm{Softmax}
\big(
s_{\text{ent}}^{(k)}
\big),
\qquad
\mathbf{q}^{(k)}
=
\mathrm{Softmax}
\big(
s_{\text{time}}^{(k)}
\big).
\]

These distributions are used to compute expected embeddings over the entity and timestamp embedding tables:
\[
\bar{\mathbf{e}}_{\text{ent}}^{(k)}
=
\sum_i
p_i^{(k)}
\mathbf{e}_i,
\qquad
\bar{\mathbf{e}}_{\text{time}}^{(k)}
=
\sum_j
q_j^{(k)}
\mathbf{t}_j.
\]

The expected entity and temporal representations are combined and projected into the latent reasoning space:
\[
\mathbf{m}^{(k)}
=
f_{\text{mem}}
\left(
\bar{\mathbf{e}}_{\text{ent}}^{(k)}
+
\bar{\mathbf{e}}_{\text{time}}^{(k)}
\right).
\]

Rather than directly replacing the current state, IMSABT-QA refines the latent representation using a memory-attention mechanism. The previous latent state attends to the memory vector through multi-head attention:
\[
\mathbf{u}^{(k)}
=
\mathrm{Attn}
\big(
\mathbf{z}^{(k-1)},
\mathbf{m}^{(k)},
\mathbf{m}^{(k)}
\big).
\]

The resulting memory-informed representation is normalized and fused with the previous state through a learned gate:
\[
\gamma^{(k)}
=
\sigma
\left(
W_g
[
\mathbf{z}^{(k-1)};
\mathbf{u}^{(k)}
]
\right),
\]
\[
\mathbf{z}^{(k)}
=
\gamma^{(k)}
\odot
\mathbf{z}^{(k-1)}
+
\big(
1-\gamma^{(k)}
\big)
\odot
\mathbf{u}^{(k)}.
\]

This recurrent working-memory update enables IMSABT-QA to iteratively refine its latent reasoning hypothesis across hops while preserving useful information from previous reasoning steps.

\subsubsection{Hop aggregation}

After completing all $K$ reasoning hops, IMSABT-QA aggregates hop-wise predictions using a learned hop-selection distribution conditioned on the global question summary:
\[
\boldsymbol{\beta}
=
\mathrm{Softmax}
\big(
W_{\text{hop}}
\mathbf{s}
\big),
\]
where
\[
\boldsymbol{\beta}
=
(\beta_1,\dots,\beta_K).
\]

The final entity and temporal prediction scores are computed as weighted combinations of the hop-specific outputs:
\[
s_{\text{ent}}
=
\sum_{k=1}^{K}
\beta_k
s_{\text{ent}}^{(k)},
\qquad
s_{\text{time}}
=
\sum_{k=1}^{K}
\beta_k
s_{\text{time}}^{(k)}.
\]

This adaptive aggregation strategy allows the model to emphasize the reasoning depth most appropriate for a given question. Questions requiring shallow reasoning may rely primarily on early hops, whereas temporally compositional or multi-step questions can place greater weight on later reasoning stages.
\subsubsection{Training objective}

IMSABT-QA is trained with cross-entropy over the concatenated entity and time score vector:
\[
\mathcal{L} = \mathrm{CE}([\mathbf{s}_{\text{ent}};\mathbf{s}_{\text{time}}], y),
\]
where $y$ is the gold answer distribution. The model therefore learns to jointly predict the correct entity or timestamp while refining its reasoning state across multiple hops.
